Optimizing Information Freshness using Low-Power Status Updates via Sleep-Wake Scheduling

In this paper, we consider the problem of optimizing the freshness of status updates that are sent from a large number of low-power source nodes to a common access point. The source nodes utilize carrier sensing to reduce collisions and adopt an asychronized sleep-wake strategy to achieve an extended battery lifetime (e.g., 10-25 years). We use age of information (AoI) to measure the freshness of status updates, and design the sleep-wake parameters for minimizing the weighted-sum peak AoI of the sources, subject to per-source battery lifetime constraints. When the sensing time is zero, this sleep-wake design problem can be solved by resorting to nested convex optimization; however, for positive sensing times, the problem is non-convex. We devise a low-complexity solution to solve this problem and prove that, for practical sensing times, the solution is within a small gap from the optimum AoI performance. Our numerical and NS-3 simulation results show that our solution can indeed elongate the batteries lifetime of information sources, while providing a competitive AoI performance.

==> sections/Discussion.tex <==
\section{Discussion}\label{Disc}
In this section, we discuss our results and compare it with prior works. 
\subsection{Preemption vs. Non-Preemption}
In the conclusion of \cite[Appendix]{CostaCodreanuEphremides_TIT}, the authors claimed that "In  the  LCFS  system  with  preemption  we  expect  that,  for  very large  arrival  rates,  the  age  would  increase  without  bound,  as  no  packet  finishes  service''. This claim is correct when the packet service times are NBU. As we will see in Fig. \ref{avg_peak_age3}, the age of the preemptive LCFS policy grows to infinity at high traffic intensity for gamma distributed service times. However, preemption does not increase the age for exponential service times, because the remaining service times of a preempted packet has the same distribution with the service time of a new packet. In Theorem \ref{thm1}, we have proven that the preemptive LCFS policy is age-optimal for exponential service times and general system parameters. In Theorem 3(a) of \cite{RYatesTIT16}, Yates and Kaul showed that the average age of the preemptive LCFS policy is a decreasing function of the traffic intensity $\rho$ in M/M/1 queues as $\rho$ grows to infinite. 

%On one hand, this contradicts our results in Theorem \ref{thm1}, in which we showed that the LCFS system with preemption can, indeed, achieve age-optimality for all arrival rates among all causal policies when the service times are exponentially distributed and the update packets arrive in the order of their generation times. Moreover, the study in \cite{RYatesTIT16} showed that the preemptive LCFS policy achieves bounded average age for all arrival rates when the service times are exponentially distributed. However, for non-exponential service time, the age of the preemptive LCFS policy could blow up at high traffic intensity (as we will see in Fig. \ref{avg_peak_age3}). This is because the packet service times are no longer memoryless. Thus, high traffic intensity leads to increased preemption rate which, in turn, leads to no packet completes service. Hence, the inter-departure times increase causing the rise in the age. From this, we can deduce that the age performance of the prmp-LGFS-R policy depends essentially on the service time distribution.

In addition, the study in \cite{Gamma_dist} characterized the age for LCFS systems with and without preemption for  gamma distributed service times. In \cite[Numerical Results]{Gamma_dist}, the authors showed that the non-preemptive LCFS policy can achieve better average age performance than the preemptive LCFS policy. In this paper, we further show that the non-prmp-LGFS-R policy is within a small constant gap from the optimum expected average age for all NBU service time distributions, which include gamma distribution as one example.

%In addition, the study in \cite{Gamma_dist} characterized the age for LCFS systems with and without preemption when the service time is gamma distributed (gamma distribution belongs to the class of NBU distributions). In \cite[Numerical Results]{Gamma_dist}, the authors showed that the non-preemptive policy can achieve better average age than the preemptive one. In this paper, we showed that the non-prmp-LGFS-R policy can come close to age-optimal when the service time is NBU distributed. More specifically, the non-prmp-LGFS-R is within a small age gap from the optimum expected average age for NBU service times.

\subsection{Replication vs. Non-Replication}
The replication technique has gained significant attention in recent years to reduce the delay in queueing systems \cite{Chen_queue_coding,yin_data_retrieve,sun2016delay}. However, under some system settings, replications may worsen the delay performance. In particular, it was shown in \cite{sun2016delay} that replication policies are far from the optimum delay for NBU service time distributions. A simple explanation of this result is as follows: Let $X_1, X_2, \ldots, X_m$ be i.i.d. NBU random variables with mean $\mathbb{E}[X_l]=\mathbb{E}[X]<\infty$. From the properties of the NBU distributions, we can obtain \cite{joshi2017efficient}
\begin{equation}\label{NBUproperty_delay}
\mathbb{E}[\min_{l=1,\ldots,m}X_l]\geq \frac{\mathbb{E}[X]}{m}.
\end{equation}
Now, if $X_l$ represents the packet service time of server $l$, then the left-hand side of \eqref{NBUproperty_delay} represents the mean service time (the mean time spent by each server per packet) when each packet is replicated to all servers; and the right-hand side of \eqref{NBUproperty_delay} represents the mean service time when there is no replication. This gives insight why packet replication can worsen the delay performance when the service time is NBU. Somewhat to our surprise, we found in this paper that the non-prmp-LGFS-R policy is near-optimal in minimizing the age, even for NBU service time distributions. The intuition behind this result is that the age is affected by the freshness of the delivered packets irrelevant to the total number of delivered packets. In other words, to reduce the age, we need to deliver the freshest packet as soon as possible. Also, it is obvious that 
\begin{equation}
\mathbb{E}[\min_{l=1,\ldots,m}X_l]\leq\mathbb{E}[X].
\end{equation}
Thus, packet replication can help in this direction by exploiting the diversity provided by multiple servers. 
\subsection{New-Worse-than-Used service time distributions}
Another important class of distributions that are more general than exponential is New-Worse-than-Used (NWU) distributions. The definition of the NWU distributions is as follows: 
\begin{definition}  \textbf{New-Worse-than-Used distributions:} Consider a non-negative random variable $Z$ with CCDF $\bar{F}(z)=\mathbb{P}[Z>z]$. Then, $Z$ is \textbf{New-Worse-than-Used (NWU)} if for all $t,\tau\geq0$
\begin{equation}\label{NWU_Inequality}
\bar{F}(\tau +t)\geq \bar{F}(\tau)\bar{F}(t).
\end{equation} 
\end{definition}
Examples of NWU distributions include hyperexponential distribution, Weibull distribution with $c <1$, etc. A  random variable is both NBU and NWU if, and only if, it is exponential. We investigated whether age-optimality can be achieved when the service times are NWU. We figured out that no policy can achieve optimality when the service times are NWU. To clarify this claim, let us consider the following example.

 \begin{figure*}[!tbp]
 \centering
 \subfigure[Case 1: Preemption is allowed.]{
  \includegraphics[scale=0.3]{figure/NWU.eps}
   \label{1a}
   }
 \subfigure[Case 2: Preemption is not allowed.]{
  \includegraphics[scale=0.3]{figure/NWU2.eps}
   \label{2b}
   }
   \caption{Illustration of policies $\pi$ and $\pi'$ in the Example }
   \label{fig:samp_path_NBU}
\end{figure*}
\textbf{Example:}
\emph{Consider a single server queue with $U(0)=0$ for all policies. We first consider the case where preemption is allowed. Suppose that the policies $\pi$ and $\pi'$ start to process packet 1 at time 0, as shown in  Fig. \ref{1a}. Suppose that at time $\delta$, packet 2 with $s_2<s_1$ arrives at the system. Since $s_1>s_2$, an intuitive action is to keep processing the fresh packet (packet 1) and ignore the old packet (packet 2). We will show that this decision may not achieve lower age. Suppose that policy $\pi'$ preempts the processing of packet 1 and starts to serve packet 2 at time $\delta$ and completes the service of packet 2 at time $\gamma$, as shown in  Fig. \ref{1a}. Let $R_1$ represent the remaining service time to complete packet 1 at time $\delta$ under policy $\pi$. Suppose that the server has spent $\chi$ ($\chi\geq 0$) seconds on processing packet 1 by time $\delta$ in policy $\pi$. Define $X_1=\chi+R_1$ as the service time of packet 1 under policy $\pi$ and $X_2=\gamma-\delta$ as the service time of packet 2 under policy $\pi'$. Then, the CCDF of $R_1$ is given by
\begin{equation}\label{ex_NWU_1}
\mathbb{P}[R_1>t]=\mathbb{P}[(X_1-\chi)>t\vert X_1>\chi].
\end{equation}
Because the packet service times are NWU, we can obtain that for all $t, \chi\geq 0$
\begin{equation}\label{ex_NWU_2}
\mathbb{P}[(X_1-\chi)>t\vert X_1>\chi]=\mathbb{P}[(X_2-\chi_1)>t\vert X_2>\chi_1]\geq\mathbb{P}[X_2>t].
\end{equation}
Combining \eqref{ex_NWU_1} and \eqref{ex_NWU_2}, we get
\begin{equation}\label{ex_NWU_3}
R_1\geq_{\text{st}}X_2.
\end{equation}
This means that the completion time of packet 2 under policy $\pi'$ is stochastically smaller than the completion time of packet 1 under policy $\pi$, as shown in  Fig. \ref{1a}. Thus, policy $\pi'$ can obtain lower age at time $\gamma$ than policy $\pi$, i.e., we have
\begin{equation}
\Delta_\pi(\gamma)=\gamma\geq\gamma-s_2=\Delta_{\pi'}(\gamma).
\end{equation}}

\emph{Now, we proceed to the case where preemption is not allowed. We will show that a non-work-conserving policy can obtain lower age than the work-conserving one. Suppose that policy $\pi$ starts processing packet 1 at time 0; and policy $\pi'$ does idle the server until time $\delta$, then assigns packet 2 to the server, as shown in Fig. \ref{2b}. We assume here that $0=a_1<a_2\leq\delta$ and $s_2>s_1$. By the same argument as in the first case, we can show that the completion time of packet 2 under policy $\pi'$ is stochastically smaller than the completion time of packet 1 under policy $\pi$, as shown in Fig. \ref{2b}. This means that the non-work-conserving policy $\pi'$ can obtain a lower age than policy $\pi$.}

This example shows that age-optimality is extremely hard to be achieved within the policy space that includes all causal policies when the service times are NWU distributed. However, we showed in \cite{multihop_optimal} that optimality can be achieved for general service time in single server queues among all non-preemptive work-conserving policies.

==> sections/Numerical_results__rahul_singh_s_conflicted_copy_2019-08-02_.tex <==
\section{Numerical Results}\label{Simulations}
Throughout, we use ``Age-optimal scheduler'' to denote the sleep-wake scheduler with the sleep period paramters $r_l^{\star}$'s as in \eqref{r_f_b_gr_1}, \textcolor{red}{that was shown to be asymptotically optimal in Theorem ?? }. By ``Throughput-optimal scheduler'', we  refer to the sleep-wake algorithm of~\cite{chen2013life} that is known to achieve the optimal trade-off between the throughput and energy consumption. Also, we use ``Fixed-rate scheduler'' to denote the \textcolor{red}{sleep-wake scheduler ??} algorithm in which the sleep period parameters $r_l$'s are equal for all the sources, i.e., $r_l=k$ for all $l$, \textcolor{red}{ where the parameter $k$ has been chosen so as to satisfy the energy constraints of Problem \textbf{1} }. \textcolor{red}{We also compare the performance of the above mentioned algorithms against the lower bounds~\eqref{lower_bound_sum_bi_ge_1}, \eqref{lower_bound_sum_bi_le_1}, and hence use the term ``lower bound'' in order to denote these lower bounds.}

\textcolor{red}{Throughout, we let the mean transmission time $\mathbb{E}[T]=5$ ms.} The weights $w_l$'s attached to different sources \textcolor{red}{refer to equation in problem } are generated by sampling from a uniform distribution in the interval $[0, 10]$. Similarly, the target energy efficiencies $b_l$'s \textcolor{red}{ of the sources\slash batteries?} are generated by sampling from the uniform distribution within the range [0, 1]. 

%The energy consumption rate for each source while it is transmitting is equal to 24.75 mW. The initial battery levels and recharging rates are set to 
%$B_l\equiv 1200$ mAh, $R_l\equiv .22$ for all sources. The target lifetimes are chosen such that the target energy efficiencies $b_l$'s are randomly generated uniformly  within the range [0, 1]. \textcolor{red}{shouldnt it be other way around? }

\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/comparison_life_add_no_users_10_vs_ration_2.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the ratio $\frac{t_s}{\mathbb{E}[T]}$ for an update system with $M=10$ sources.}
%\vspace{-.1in}
\label{peak_age_comp}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/comparison_life_add_vs_no_users.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the number of sources $M$.}
%\vspace{-.1in}
\label{peak_age_comp_num}
\end{figure}
We set the number of sources at $M=10$. 
Fig.~\ref{peak_age_comp} plots the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ ~\eqref{t_avg_peak_age} as a function of the ratio $\frac{t_s}{\mathbb{E}[T]}$. The age-optimal scheduler is seen to outperform the throughput-optimal and fixed-rate schedulers. This is not surprising since the throughput-optimal had been designed in order to maximize the throughput, and not minimize the age.
Moreover, we also observe that the \textcolor{red}{performance} of the age-optimal scheduler converges to the lower bound as $t_s/\mathbb{E}[T]\to 0$. \textcolor{red}{This is in accordance with our result on the near-optimality of } \textcolor{red}{what ?}. Finally, we observe that the total weighted average peak age of all schedulers increases as the sensing time increases. This is \textcolor{red}{expected since an increase in the sensing time leads to an increase in the probability of packet collisions, which in turn increases the average age.}



We then scale the number of sources $M$, and plot $\bar{\Delta}^{\text{peak}}$ as a function of $M$ in Fig.~\ref{peak_age_comp_num}. The sensing time $t_s$ is fixed at $t_s=40~\mu$s. The age-optimal scheduler is shown to outperform the other schedulers uniformly for all values of $M$. As expected, the total weighted average peak age of each scheduler increases with $M$, \textcolor{red}{ since...why??}. The gap between \textcolor{red}{the performance of age-optimal scheduler and the lower bound increases with $M$}. \textcolor{red}{This is the case because, as shown in equation ??, the sub-optimality gap is a linear increasing function of the parameters $C_1$,$C_2$~\eqref{eq23thm3_1} and \eqref{eq29thm3_3}, and moreover $C_1,C_2$ are increasing functions of $M$.}

%As we can observe, our proposed sleep-wake algorithm outperforms the other two algorithms in both the cases. This is not surprising since the ``Life-add'' algorithm \textcolor{red}{of paper name..} was designed to maximize the throughput, and optimizing the throughput does not translate to optimizing the AoI. Moreover, in Figure \ref{peak_age_comp}, we observe that the total weighted average peak age for all algorithms increases as the sensing time increases. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collisions, and hence the age performances of these \textcolor{red}{is it all these algos?} algorithms deteriorate.

%while using the sleep-wake algorithm, we will set the rate parameters $r_l$ as in \eqref{r_f_b_gr_1}.
%We compare the performance of our proposed sleep-wake algorithm with the round robin \cite{li2013throughput,hsu2017scheduling,kadota2016minimizing,kadota2016minimizing_journal,jiang2018timely}. Under the round robin algorithm sources take turns in order to transmit their update packet. Thus, once a source obtains channel access, it transmits until its battery dies out. The execution of an algorithm is completed when all the sources run out of their battery energy. To keep comparisions fair, in case the execution of an algorithm completes before the other, its peak age still gets updated even though it is known that it would not be transmitting packets at future time instants. \par
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.4]{figure/rr_vs_swc_weights_5_1_,1.eps}
%\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
%\caption{Total weighted average peak age $\bar{\Delta}^p$ versus the ratio $\frac{t_s}{\mathbb{E}[T]}$ for an update system with $M=3$ sources.}
%%\vspace{-.1in}
%\label{peak_age_comp}
%\end{figure}
%\begin{table}[t]
%\footnotesize
% \centering
%\begin{tabular}{|l|l|l|l|}
%\hline
%Source & Weight & \begin{tabular}[c]{@{}l@{}}Initial battery \\ level (in mAh)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Target lifetime\\ (in hours)\end{tabular} \\ \hline
%Source 1 & 5 & 500 & 33.7 \\ \hline
%Source 2 & 1 & 1000 & 134.7 \\ \hline
%Source 3 & 0.1 & 1200 & 242.4 \\ \hline
%\end{tabular}
%\caption{Parameters of the heterogeneous sources.}
%\label{tab:my-table}
%\end{table}
%We first consider an information-update system with $M=3$ sources. We suppose that
%the transmission times are deterministic, i.e., $T_i= T=5$ ms for all $i$. Figure \ref{peak_age_comp} plots the total weighted average peak age $\bar{\Delta}^p$ versus the ratio $\frac{t_s}{T}$. The energy consumption rate for each source while it is transmitting, is equal to 24.75 mW. The weights $w_l$'s associated with various sources, their initial battery levels $B_l$'s, and target lifetimes $D_l$'s are as in Table \ref{tab:my-table}. As observed in Fig.~\ref{peak_age_comp} , the proposed sleep-wake algorithm outperforms the round robin for small values of $\frac{t_s}{\mathbb{E}[T]}$. This is because when the sensing time decreases, the probability of packet collision decreases. Moreover, our algorithm provides a near optimal trade-off between minimizing the AoI and energy consumption when the ratio $\frac{t_s}{T}$ is small. However, as we can see, the round robin algorithm outperforms our proposed sleep-wake algorithm for high values of $\frac{t_s}{T}$. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collision, and hence the age performance of the sleep-wake algorithm deteriorates. 



\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/age_with_lower_bound_vs_energy_2.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the target energy efficiency $b$ for an update system with $M=10$ sources.}
%\caption{Total weighted average peak age $\bar{\Delta}^p$ versus the target lifetime $D$ for an update system with $M=10$ sources.}
%\vspace{-.1in}
\label{peak_age_comp_lower_bound}
\end{figure}

We now fix the value of $M$ at $10$ sources and the target energy efficiencies at the same value for all the sources, i.e., $b_l\equiv b$. We then vary the parameter $b$ and plot the resulting performances in Fig.~\ref{peak_age_comp_lower_bound}. We exclude simulations for $b< 0.1$ since the scheme of~\cite{chen2013life} is infeasible for Problem \textbf{1}. The age-optimal scheduler outperforms the rest of the schedulers and its performance is very close to the lower bound. Its performance is a decreasing function of $b$, and eventually settles at a constant value. This plot agrees with our analysis since from~\eqref{r_f_b_gr_1} we observe that there exists a value for $b$ after which our proposed solution value \textcolor{red}{is it $r^\star$??} is a function solely of weights $w_l$'s and $\beta^\star$, and not of $b$. Thus, unsurprisingly, the performance of the proposed scheduler saturates after this value of $b$. 










%We now consider an information-update system with $M=10$ sources. The target lifetimes of all the sources are taken to be the same, i.e., $D_l=D$ for all $l$. Figure \ref{peak_age_comp_lower_bound} plots the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ versus the target lifetime $D$.
%% The mean of the packet transmission times is $\mathbb{E}[T]=5$ ms. 
%%The sensing time is $t_s=40~\mu$s. 
%%The energy consumption in a transmission mode is 24.75 mW.
% We consider homogeneous sources, where weight $w_l=1$, and initial battery level $B_l=300$ mAh, for all $l$. 
%The ``Lower bound” curve is generated from the lower bounds in \eqref{lower_bound_final_sumbi_ge1} and \eqref{lower_bound_72} in Appendix \ref{Appendix_A} that are constructed to solve Problem \textbf{1} and \textbf{2}. As we can observe, the total weighted average peak age increases as the target lifetime increases. This is because, as the target lifetime increases, our proposed sleep-wake algorithm reduces the packet transmission rate of the sources in order to meet the target lifetimes (or equivalently the energy constraints\textcolor{red}{equation number and is it battery?}), and hence AoI increases. We also observe that the total weighted average peak age of our proposed policy coincides with the lower bounds derived in\textcolor{red}{equation number?}. This is not surprising since the proposed sleep-wake algorithm is near age optimal in the regime when the ratio of the carrier sensing time to the mean transmission time ($\frac{t_s}{\mathbb{E}[T]}$) is small, which is .008 in this case. 
%%The plot also confirms that the bounds~\eqref{lower_bound_final_sumbi_ge1} and \eqref{lower_bound_72} are tight.

==> sections/Numerical_results_old.tex <==
\section{Numerical Results}\label{Simulations}
Throughout, we use ``Age-optimal scheduler'' to denote the sleep-wake scheduler with the sleep period paramters $r_l^{\star}$'s as in \eqref{r_f_b_gr_1}, which was shown to be near-optimal in Theorem \ref{thm_case_sum_bi_ge_1} and Theorem \ref{thm_case_sum_bi_le_1}. By ``Throughput-optimal scheduler'', we  refer to the sleep-wake algorithm of~\cite{chen2013life} that is known to achieve the optimal trade-off between the throughput and energy consumption. Also, we use ``Fixed-rate scheduler'' to denote the sleep-wake scheduler in which the sleep period parameters $r_l$'s are equal for all the sources, i.e., $r_l=k$ for all $l$ such that $k$ is chosen to satisfy the energy constraints in Problem \textbf{1}. Finally, the ``Lower bound'' curves are generated from the lower bounds in \eqref{lower_bound_sum_bi_ge_1} and \eqref{lower_bound_sum_bi_le_1}.

Unless stated otherwise, our setups are as follows: The average transmission time is $\mathbb{E}[T]=5$ ms. The weights $w_l$'s attached to different sources are generated by sampling from a uniform distribution in the interval $[0, 10]$. The target energy efficiencies $b_l$'s are randomly generated uniformly  within the range [0, 1]. 

%The energy consumption rate for each source while it is transmitting is equal to 24.75 mW. The initial battery levels and recharging rates are set to 
%$B_l\equiv 1200$ mAh, $R_l\equiv .22$ for all sources. The target lifetimes are chosen such that the target energy efficiencies $b_l$'s are randomly generated uniformly  within the range [0, 1]. \textcolor{red}{shouldnt it be other way around? }

\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/comparison_life_add_no_users_10_vs_ration_2.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the ratio $\frac{t_s}{\mathbb{E}[T]}$ for an update system with $M=10$ sources.}
%\vspace{-.1in}
\label{peak_age_comp}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/comparison_life_add_vs_no_users.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the number of sources $M$.}
%\vspace{-.1in}
\label{peak_age_comp_num}
\end{figure}
Figures \ref{peak_age_comp} plot the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ in \eqref{t_avg_peak_age} versus the ratio $\frac{t_s}{\mathbb{E}[T]}$.  We consider an information-update system with $M=10$ sources. As we can observe, the age-optimal scheduler outperforms the throughput-optimal and fixed-rate schedulers. This implies that what minimizes the throughput does not necessary minimize AoI and vice versa. Moreover, we can observe that the total weighted average peak age of the age-optimal scheduler converges to the lower bound as $t_s/\mathbb{E}[T]\to 0$. This agrees with our near-optimal results. Finally, we observe that the total weighted average peak age of all schedulers increases as the sensing time increases. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collisions, and hence the age performances of these schedulers deteriorate.



Figures  \ref{peak_age_comp_num} plot the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ in \eqref{t_avg_peak_age} versus the number of sources $M$.   We set the sensing time to be $t_s=40~\mu$s. Again, we observe that the age-optimal scheduler outperforms the throughput-optimal and fixed-rate schedulers. Moreover, the total weighted average peak age of all schedulers increases with the number of sources, which is reasonable. Beside that, the gap between total weighted average peak age of age-optimal scheduler and the lower bound curve increase with the number of source. This is because the gap is a linearly increasing function of $C_1$ and $C_2$ in \eqref{eq23thm3_1} and \eqref{eq29thm3_3}, respectively, which increase with the number of sources. 

%As we can observe, our proposed sleep-wake algorithm outperforms the other two algorithms in both the cases. This is not surprising since the ``Life-add'' algorithm \textcolor{red}{of paper name..} was designed to maximize the throughput, and optimizing the throughput does not translate to optimizing the AoI. Moreover, in Figure \ref{peak_age_comp}, we observe that the total weighted average peak age for all algorithms increases as the sensing time increases. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collisions, and hence the age performances of these \textcolor{red}{is it all these algos?} algorithms deteriorate.

%while using the sleep-wake algorithm, we will set the rate parameters $r_l$ as in \eqref{r_f_b_gr_1}.
%We compare the performance of our proposed sleep-wake algorithm with the round robin \cite{li2013throughput,hsu2017scheduling,kadota2016minimizing,kadota2016minimizing_journal,jiang2018timely}. Under the round robin algorithm sources take turns in order to transmit their update packet. Thus, once a source obtains channel access, it transmits until its battery dies out. The execution of an algorithm is completed when all the sources run out of their battery energy. To keep comparisions fair, in case the execution of an algorithm completes before the other, its peak age still gets updated even though it is known that it would not be transmitting packets at future time instants. \par
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.4]{figure/rr_vs_swc_weights_5_1_,1.eps}
%\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
%\caption{Total weighted average peak age $\bar{\Delta}^p$ versus the ratio $\frac{t_s}{\mathbb{E}[T]}$ for an update system with $M=3$ sources.}
%%\vspace{-.1in}
%\label{peak_age_comp}
%\end{figure}
%\begin{table}[t]
%\footnotesize
% \centering
%\begin{tabular}{|l|l|l|l|}
%\hline
%Source & Weight & \begin{tabular}[c]{@{}l@{}}Initial battery \\ level (in mAh)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Target lifetime\\ (in hours)\end{tabular} \\ \hline
%Source 1 & 5 & 500 & 33.7 \\ \hline
%Source 2 & 1 & 1000 & 134.7 \\ \hline
%Source 3 & 0.1 & 1200 & 242.4 \\ \hline
%\end{tabular}
%\caption{Parameters of the heterogeneous sources.}
%\label{tab:my-table}
%\end{table}
%We first consider an information-update system with $M=3$ sources. We suppose that
%the transmission times are deterministic, i.e., $T_i= T=5$ ms for all $i$. Figure \ref{peak_age_comp} plots the total weighted average peak age $\bar{\Delta}^p$ versus the ratio $\frac{t_s}{T}$. The energy consumption rate for each source while it is transmitting, is equal to 24.75 mW. The weights $w_l$'s associated with various sources, their initial battery levels $B_l$'s, and target lifetimes $D_l$'s are as in Table \ref{tab:my-table}. As observed in Fig.~\ref{peak_age_comp} , the proposed sleep-wake algorithm outperforms the round robin for small values of $\frac{t_s}{\mathbb{E}[T]}$. This is because when the sensing time decreases, the probability of packet collision decreases. Moreover, our algorithm provides a near optimal trade-off between minimizing the AoI and energy consumption when the ratio $\frac{t_s}{T}$ is small. However, as we can see, the round robin algorithm outperforms our proposed sleep-wake algorithm for high values of $\frac{t_s}{T}$. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collision, and hence the age performance of the sleep-wake algorithm deteriorates. 



\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/age_with_lower_bound_vs_energy_2.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the target energy efficiency $b$ for an update system with $M=10$ sources.}
%\caption{Total weighted average peak age $\bar{\Delta}^p$ versus the target lifetime $D$ for an update system with $M=10$ sources.}
%\vspace{-.1in}
\label{peak_age_comp_lower_bound}
\end{figure}
In Figure \ref{peak_age_comp_lower_bound}, we consider an information-update system with $M=10$ sources, where   the target energy efficiency of all sources are taken to be the same, i.e., $b_l=b$ for all $l$. Figure \ref{peak_age_comp_lower_bound} plots the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ in \eqref{t_avg_peak_age} versus the target energy efficiency $b$. We can observe that, we start our simulation from the point $b=0.1$. This is because, in enegry-scarce regime, i.e., when $\sum_{i=1}^Mb_i<1$, the sleeping period parameters that are proposed in \cite{chen2013life} are not feasible for Problem \textbf{1}, and hence we cannot compare our proposed scheduler with the throughput-optimal scheduler in this case. We can observe that the age-optimal scheduler outperforms the throughput-optimal and fixed-rate schedulers and its total weighted average peak age comes close to the lower bound curve. Moreover, as the target efficiency $b$ increases, the total weighted average peak age of age-optimal scheduler decreases and then saturates. To understand this behavior, let us recall our proposed solution in \eqref{r_f_b_gr_1}. We can observe that there exists a value for $b$ after which our proposed solution value depends only on the weights $w_l$'s and $\beta^\star$ and does not depend on $b$. That is way, the age performance of our proposed scheduler saturates after this point. 










%We now consider an information-update system with $M=10$ sources. The target lifetimes of all the sources are taken to be the same, i.e., $D_l=D$ for all $l$. Figure \ref{peak_age_comp_lower_bound} plots the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ versus the target lifetime $D$.
%% The mean of the packet transmission times is $\mathbb{E}[T]=5$ ms. 
%%The sensing time is $t_s=40~\mu$s. 
%%The energy consumption in a transmission mode is 24.75 mW.
% We consider homogeneous sources, where weight $w_l=1$, and initial battery level $B_l=300$ mAh, for all $l$. 
%The ``Lower bound” curve is generated from the lower bounds in \eqref{lower_bound_final_sumbi_ge1} and \eqref{lower_bound_72} in Appendix \ref{Appendix_A} that are constructed to solve Problem \textbf{1} and \textbf{2}. As we can observe, the total weighted average peak age increases as the target lifetime increases. This is because, as the target lifetime increases, our proposed sleep-wake algorithm reduces the packet transmission rate of the sources in order to meet the target lifetimes (or equivalently the energy constraints\textcolor{red}{equation number and is it battery?}), and hence AoI increases. We also observe that the total weighted average peak age of our proposed policy coincides with the lower bounds derived in\textcolor{red}{equation number?}. This is not surprising since the proposed sleep-wake algorithm is near age optimal in the regime when the ratio of the carrier sensing time to the mean transmission time ($\frac{t_s}{\mathbb{E}[T]}$) is small, which is .008 in this case. 
%%The plot also confirms that the bounds~\eqref{lower_bound_final_sumbi_ge1} and \eqref{lower_bound_72} are tight.

==> sections/learning.tex <==
\section{Learning}\label{sec:learning}
The algorithms derived in the previous sections assumed that the users had knowledge of the sensing time $t_s$ and average transmission time $\mathbb{E}[T]$. However, in real-world applications, the transmission and sensing times of users depend upon the surrounding environments, and hence such an assumption is not justified. In this section we assume that $t_s,\mathbb{E}[T]$ are unknown and the goal is to devise an algorithm that ``learns" them in order to use the estimates for solving~\eqref{problem1}. We will only be interested in finite sample guarantees, i.e., what performance guarantees can be provided when the learning algorithm uses only finitely many samples for estimating  $\mathbb{E}[T]$.

Let $\hat{\mathbb{E}}[T]$ denote the estimate of $\mathbb{E}[T]$ from $N$ transmission times samples $\{ T_i \}_{i=1}^{N}$,
\begin{align}\label{eq:est_T}
\hat{\mathbb{E}}[T]:= \frac{\sum_{i=1}^{N} T_i}{N(t)}.
\end{align} 
It then follows that 
\begin{align}\label{eq:chernoff}
\mathbb{P}\left( |\hat{\mathbb{E}}[T] - \mathbb{E}[T] |>\epsilon \right) \leq e^{-N\epsilon^2 }.
\end{align}
Let $\hat{r}^{\star}_{l}(t)$ denote an estimate of the optimal rates obtained by plugging in the estimate $\hat{\mathbb{E}}[T]$ in the relation~\eqref{r_f_b_gr_1}.
\footnote{Note that since the average transmission time is common to all users, the estimate $\hat{\mathbb{E}}[T](t)$ can be calculated by the AP if the users communicate their transmission times to it.}
\begin{lemma}\label{lemma:learn_1}
Let $\epsilon,\delta>0$ be user-provided parameters. If the number of samples $N$ used to estimate the transmission time is larger than $N(\epsilon,\delta):= \frac{ \log(1\slash \delta )  }{\epsilon^2}$, then 
\begin{align}\label{eq:chernoff_1}
\mathbb{P}\left( |\hat{\mathbb{E}}[T] - \mathbb{E}[T] |>\epsilon \right) \leq \delta .
\end{align}
Consequently, for values of $N$ larger than $N(\epsilon,\delta)$, we have
\begin{align}\label{eq:chernoff_2}
\mathbb{P}\left( |\hat{r}^{\star}_{l}- \hat{r}^{\star}_{l} |>\kappa \epsilon \right) \leq \delta,
\end{align}
where $\kappa = $.
\end{lemma}
Since with a high probability the estimate $\mathbf{\hat{r}}^{\star}$ is close to the true optima $\mathbf{r}^{\star}$, we would expect the average age incurred by using $\mathbf{\hat{r}}^{\star}$ should be nearly optimal. This is shown next.

\emph{Performance Analysis of CSMA under $\mathbf{\hat{r}}^{\star}$}\\ 
In order to analyze the evolution of ages of users in the CSMA system, we will sample the continuous-time process at time instants when either a packet transmission or a packet collision occurs.~This gives us an equivalent \emph{discrete-time} Markov chain in which the state of the system at time $t$, denoted $\mathbf{x}(t)$ is equal to the age values of all the users. We notice that the state-space is equal to $\mathbb{R}^{M}$, and hence is uncountable and non-compact. This is in departure with the existing works in the machine learning community~\cite{DBLP:journals/ftml/BubeckC12} which restrict the study of learning algorithms solely to discrete, finite spaces. 

Denote the transition probability kernel of the Markov chain $\mathbf{x}(t)$ by $P_{\mathbf{r}}( \mathbf{y} | \mathbf{x} )$, where the sub-script denotes its dependence upon the rate vector $\mathbf{r}$. Consider $M$ exponentially distributed random variables.

The transition probabilities are described as
\begin{align*}
P_{\mathbf{r}}( \mathbf{y} | \mathbf{x} ) = q \left(\mathbf{x} + \mathbf{1} \mathcal{R}_1 \right) + \sum_{i=1}^{M} p_i \left(   \right)
\end{align*}
where $p_1$
\textbf{Note:Verify from Ahmed}: only two events can occurr:\\
a) min r + service time, if collision\\
b) if no collision then min r becomes equal to service time and the remaining increase by min r + service time.


Let $V_{t}(\mathbf{x})$ denote the cumulative average age incurred by the system starting in age $\mathbf{x}$ and evolving for time-duration $t$ under the rate vector set equal to $\mathbf{r}$. Similarly $\tilde{V}_{t}(\mathbf{x})$



\begin{lemma}\label{lemma:learn_2}
Consider CSMA rate vectors $\mathbf{r},\mathbf{\tilde{r}}$ that satisfy 
\begin{align}\label{eq:condit_1}
|P_{\mathbf{r}}( \cdot | \mathbf{x} ) - P_{\mathbf{\tilde{r}}}( \cdot | \mathbf{x} ) | \leq \epsilon P_{\mathbf{r}}( \cdot | \mathbf{x} ), \forall \mathbf{x}.
\end{align}  
Then,
\begin{align*}
| V_t(\mathbf{x}) - \tilde{V}_t(\mathbf{x})   | \leq \epsilon V_t(\mathbf{x}).
\end{align*}
\end{lemma}
\proofname \\We have
\begin{align*}
V_{t+1}(\mathbf{x}) & =  C_{t+1}( \mathbf{x} ) + \int_{\mathbf{y}} V_{t}(\mathbf{x}) P_{\mathbf{r}}( \mathbf{y} | \mathbf{x} ) \mathrm{d} \mathbf{x} \\
\tilde{V}_{t+1}(\mathbf{x}) & =  C_{t+1}( \mathbf{x} ) + \int_{\mathbf{y}} \tilde{V}_t(\mathbf{x})  P_{\mathbf{\tilde{r}}}( \mathbf{y} | \mathbf{x} ) \mathrm{d} \mathbf{x}.
\end{align*}
Subtracting the above equalities for $t=0$ yields
\begin{align*}
| V_1(\mathbf{x}) - \tilde{V}_1(\mathbf{x}) |  = \epsilon \bar{V}_{0}(\mathbf{x}). 
\end{align*}
Now assume we have $| V_{t}(\mathbf{x}) - \tilde{V}_{t}(\mathbf{x}) |   \leq  \epsilon c_t t$.

For times $t\neq 1$, subtracting the two equations, we obtain
\begin{align}\label{eq:backward_recursion}
| V_{t+1}(\mathbf{x}) - \tilde{V}_{t+1}(\mathbf{x}) | & \leq  \epsilon \bar{V}_{t}(\mathbf{x}) + \int |V_t(\mathbf{y}) - \tilde{V}_{t}(\mathbf{y}) |    P_{\mathbf{r}}( \mathbf{y} | \mathbf{x} ) \mathrm{d} \mathbf{x}\notag\\
&\leq \epsilon M t + c_t \epsilon t \notag\\
&= (M + c_t) \epsilon t,
\end{align}
and hence the coefficients $c_t$ satisfy the recursion
\begin{align*}
c_{t+1} = M + c_t,
\end{align*}
so that $C_T = M T$, and hence $| V_{T}(\mathbf{x}) - \tilde{V}_{T}(\mathbf{x}) |\leq MT $. Dividing the inequality by time $T$, we obtain the desired result.

\begin{theorem}\label{th:pac_bound}
The average peak age performance under the CSMA swc using $\mathbf{\hat{r}}^{\star}$ is within $\epsilon M$ of the optimal performance.
\end{theorem}

